SLYKLatent: A Learning Framework for Gaze Estimation Using Deep Facial Feature Learning

In this research, we present SLYKLatent, a novel approach for enhancing gaze estimation by addressing appearance instability challenges in datasets due to aleatoric uncertainties, covariant shifts, and test domain generalization. SLYKLatent utilizes Self-Supervised Learning for initial training with facial expression datasets, followed by refinement with a patch-based tri-branch network and an inverse explained variance-weighted training loss function. Our evaluation on benchmark datasets achieves a 10.9% improvement on Gaze360, supersedes top MPIIFaceGaze results with 3.8%, and leads on a subset of ETH-XGaze by 11.6%, surpassing existing methods by significant margins. Adaptability tests on RAF-DB and Affectnet show 86.4% and 60.9% accuracies, respectively. Ablation studies confirm the effectiveness of SLYKLatent's novel components.

==> bio.tex <==
\begin{document}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.8in,clip,keepaspectratio]{bio/Samuel-bio.pdf}}]{Samuel Adebayo}
earned a First Class BSc in Electronic and Computer Engineering from Lagos State University, Lagos Nigeria (2016-2020) and is currently pursuing his PhD in Machine Learning at Queen's University Belfast, UK (2020-2024). Samuel's research is deeply rooted in computational intelligence, with a primary focus on the intricate dynamics of human hand-eye coordination and its implications for human-robot interactions. This aligns with his broader interest in advancing the fields of Computer Vision, Deep Learning, Natural Language Processing, and Bayesian Machine Learning. Beyond academics, Samuel transitioned from his role as the branch chair of the IEEE Student Branch at Lagos State University to his current leadership position as the Student Branch Chair at Queen's University Belfast.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.8in,clip,keepaspectratio]{bio/Joost-bio.pdf}}]
{Joost C. Dessing} received MSc. And PhD degrees in Human Movement Sciences from Vrije University Amsterdam, Amsterdam, The Netherlands, in 2001 and 2005, respectively.
He is currently a Lecturer at the School of Psychology of Queen's University Belfast, where he co-directs the Science in Motion lab. His research interests are fundamental and applied instances of eye-hand coordination, with a particular focus on sports and manufacturing scenarios. He studies these using 3D motion tracking, virtual reality, and neurophysiological tools.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.8in,clip,keepaspectratio]{bio/Seán-bio.pdf}}]
{Se\'an McLoone} (S$'94$ -- M$'88$  -- SM$'02$) received an M.E. degree in Electrical and Electronic Engineering and a PhD in Control Engineering from Queen's University Belfast, Belfast, U.K. in 1992 and 1996, respectively.
He is currently a Professor and Director of the Energy Power and Intelligent Control Research Centre at Queen's University Belfast. His research interests are in Applied Computational Intelligence and Machine Learning with a particular focus on data based modelling and analysis of dynamical systems, with applications in advanced manufacturing informatics, energy and sustainability, connected health and assisted living technologies.
Prof. McLoone is a Chartered Engineer and Fellow of the Institution of Engineering and Technology. He is a Past Chairman of the UK and Republic of Ireland (UKRI) Section of the IEEE.
\end{IEEEbiography}
\end{document}
